Interval Observer of Minimal Error Dynamics

This paper proposes a simple interval observer which can generate tighter interval estimates of variables in transient states than the standard interval observer. The simple nonlinear dynamics shrinks the estimated intervals to true state variables at the maximum velocity in the absence of disturbances. In the presence of bounded disturbances, ultimate bounded of the interval estimates are given under the standard assumption for interval observer design.

==> fig11x1.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m11i5f5d8x1_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_1. \overline{x}_1]$ estimated by
the standard interval observer with the single gain $G_1$. 
}
\label{fig:11x1}
%\vspace{2ex}
\end{figure}


==> fig11x2.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m11i5f5d8x2_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_2. \overline{x}_2]$ estimated by
the standard interval observer with the single gain $G_1$. 
}
\label{fig:11x2}
%\vspace{2ex}
\end{figure}


==> fig13x1.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m13i5f5d8x1_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_1. \overline{x}_1]$ estimated by 
the proposed interval observer 
\eqref{eq:mintobs} with the three gains \eqref{eq:exL123}. 
}
\label{fig:13x1}
%\vspace{2ex}
\end{figure}


==> fig13x2.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m13i5f5d8x2_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_2. \overline{x}_2]$ estimated by 
the proposed interval observer 
\eqref{eq:mintobs} with the three gains \eqref{eq:exL123}. 
}
\label{fig:13x2}
%\vspace{2ex}
\end{figure}


==> fig22x1.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m22i5f5d8x1_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_1. \overline{x}_1]$ estimated by 
the standard interval observer with the single gain $G_2$. 
}
\label{fig:22x2}
%\vspace{2ex}
\end{figure}


==> fig22x2.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m22i5f5d8x2_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_2. \overline{x}_2]$ estimated by
the standard interval observer with the single gain $G_2$. 
}
\label{fig:22x2}
%\vspace{2ex}
\end{figure}


==> fig33x1.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m33i5f5d8x1_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_1. \overline{x}_1]$ estimated by
the standard interval observer with the single gain $G_3$. 
}
\label{fig:33x1}
%\vspace{2ex}
\end{figure}


==> fig33x2.tex <==
\begin{figure}[t]
%\hspace{-1ex}%
\begin{tabular}{c}
\includegraphics[width=7.5cm,height=5.5cm]{miiobsmplt_4m33i5f5d8x2_c}
\\
\end{tabular}
\caption{The state variable $x_3$ and the interval 
$[\underline{x}_2. \overline{x}_2]$ estimated by
the standard interval observer with the single gain $G_3$. 
}
\label{fig:33x2}
%\vspace{2ex}
\end{figure}

